Lifetime effects and satellites in the photoelectron spectrum of platinum metal

This work presents a comprehensive investigation of the electronic structure and many-body photoemission effects in metallic platinum using reflection high-energy electron energy-loss spec- troscopy (RHEELS), soft X-ray photoelectron spectroscopy (SXPS), and hard X-ray photoelectron spectroscopy (HAXPES), supported by ab initio calculations. Shallow and deep core state spectra enable the systematic characterisation of intrinsic line-shape asymmetries and satellite structures. Correlation of photoelectron satellites with RHEELS loss features allows the assignment of inter- band transitions, surface and bulk plasmons, plasmonic overtones, and semi-core ionisation losses across the Pt spectrum. Several previously unresolved satellite features and spin-orbit splittings are identified and discussed. Comparison of experimental valence band spectra with orbital-projected densities of states calculated using ab initio density functional theory (DFT) and G0W0 approaches, with and without spin-orbit coupling, demonstrates the critical role of relativistic effects in reproducing the Pt valence electronic structure. Together, these results establish a unified, internally consistent spectroscopic reference for metallic platinum, providing a robust framework for interpreting photoelectron spectra of Pt-containing catalysts, electronic materials, and related 5d transition metal systems.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
